Probing spin-dependent dark matter interactions with $^6$Li

CRESST is one of the most prominent direct detection experiments for dark matter particles with sub-GeV/c$^2$ mass. One of the advantages of the CRESST experiment is the possibility to include a large variety of nuclides in the target material used to probe dark matter interactions. In this work, we discuss in particular the interactions of dark matter particles with protons and neutrons of $^{6}$Li. This is now possible thanks to new calculations on nuclear matrix elements of this specific isotope of Li. To show the potential of using this particular nuclide for probing dark matter interactions, we used the data collected previously by a CRESST prototype based on LiAlO$_2$ and operated in an above ground test-facility at Max-Planck-Institut f\"ur Physik in Munich, Germany. In particular, the inclusion of $^{6}$Li in the limit calculation drastically improves the result obtained for spin-dependent interactions with neutrons in the whole mass range. The improvement is significant, greater than two order of magnitude for dark matter masses below 1 GeV/c$^2$, compared to the limit previously published with the same data.

==> authorss.tex <==

\author
{%
G.~Angloher\thanksref{addr1}\and
S.~Banik\thanksref{addr7}\and
G.~Benato\thanksref{addr13}\and
A.~Bento\thanksref{addr1,addr2}\and
E.~Bertoldo\thanksref{t1,e1,addr1}\and
A.~Bertolini\thanksref{addr1} \and
R.~Breier\thanksref{addr13}\and
C.~Bucci\thanksref{addr3}\and
L.~Canonica\thanksref{addr1}\and
A.~D'Addabbo\thanksref{addr3,addr10}\and
S.~Di~Lorenzo\thanksref{addr3,addr10}\and
L.~Einfalt\thanksref{addr7}\and
A.~Erb\thanksref{addr4,addr5}\and
F.~v.~Feilitzsch\thanksref{addr4}\and
N.~Ferreiro~Iachellini\thanksref{addr1,addr16}\and
S.~Fichtinger\thanksref{addr7}\and
D.~Fuchs\thanksref{addr1}\and
A.~Fuss\thanksref{addr7,addr8}\and
V.M.~Ghete\thanksref{addr7,addr8}\and
A.~Garai\thanksref{addr1}\and
P.~Gorla\thanksref{addr3}\and
D.~Hauff\thanksref{addr1}\and
M. Je\v{s}kovsk\'{y}\thanksref{addr13}\and
J.~Jochum\thanksref{addr6}\and
M.~Kaznacheeva\thanksref{addr4}\and
A.~Kinast\thanksref{addr4}\and
H.~Kluck\thanksref{addr7,addr8}\and
H.~Kraus\thanksref{addr9}\and 
A.~Langenk\"amper\thanksref{addr4}\and
M.~Mancuso\thanksref{t1,e2,addr1}\and
L.~Marini\thanksref{addr13}\and
V.~Mokina\thanksref{addr7}\and
A.~Nilima\thanksref{addr1} \and
M.~Olmi\thanksref{addr3,addr10}\and
T.~Ortmann\thanksref{addr4}\and
C.~Pagliarone\thanksref{addr3,addr11}\and
V. Palu\v{s}ov\'a\thanksref{addr13}\and
L.~Pattavina\thanksref{addr3,addr4}\and
F.~Petricca\thanksref{addr1}\and
W.~Potzel\thanksref{addr4}\and
P.~Povinec\thanksref{addr13}\and
F.~Pr\"obst\thanksref{addr1}\and
F.~Pucci\thanksref{addr1} \and
V.~Palu\v{s}ov\'a\thanksref{addr13}\and
F.~Reindl\thanksref{addr7,addr8}\and
J.~Rothe\thanksref{addr1,addr3}\and
K.~Sch\"affner\thanksref{addr1}\and
J.~Schieck\thanksref{addr7,addr8}\and
V.~Schipperges\thanksref{addr6}\and
D.~Schmiedmayer\thanksref{addr7,addr8}\and
S.~Sch\"onert\thanksref{addr4}\and
C.~Schwertner\thanksref{addr7,addr8}\and
M.~Stahlberg\thanksref{addr1}\and
L.~Stodolsky\thanksref{addr1}\and
C.~Strandhagen\thanksref{addr6}\and
R.~Strauss\thanksref{addr4}\and
I.~Usherov\thanksref{addr6}\and 
F.~Wagner\thanksref{addr7,addr8}\and 
M.~Willers\thanksref{addr4}\and
V.~Zema\thanksref{addr3,addr10,addr15}\and
(The CRESST Collaboration)\\
}


%
%
%
%
\institute
{%
Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany 
\label{addr1} \and
Comenius University, Faculty of Mathematics, Physics and Informatics, SK-84248 Bratislava, Slovakia
\label{addr13}\and
INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy 
\label{addr3} \and
Physik-Department and Excellence Cluster Universe, Technische Universit\"at M\"unchen, D-85748 Garching, Germany 
\label{addr4} \and
Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, A-1050 Wien, Austria 
\label{addr7} \and
Atominstitut, Vienna University of Technology, A-1020 Wien, Austria 
\label{addr8} \and
Eberhard-Karls-Universit\"at T\"ubingen, D-72076 T\"ubingen, Germany 
\label{addr6} \and
Department of Physics, University of Oxford, Oxford OX1 3RH, United Kingdom 
\label{addr9} \and
also at: Departamento de Fisica, Universidade de Coimbra, P3004 516 Coimbra, Portugal 
\label{addr2} \and
also at: GSSI-Gran Sasso Science Institute, 67100, L'Aquila, Italy 
\label{addr10} \and
also at: Walther-Mei{\ss}ner-Institut f\"ur Tieftemperaturforschung, D-85748 Garching, Germany 
\label{addr5} \and
also at: LIBPhys, Dipartimento di Ingegneria Civile e Meccanica, Universit\`{a} degli Studi di Cassino e del Lazio Meridionale, I-03043 Cassino, Italy 
\label{addr11} \and
also at: Chalmers University of Technology, Department of Physics, SE-412 96 G\"oteborg, Sweden 
\label{addr15} \and
also at: Exzellenzcluster ORIGINS, Garching, Germany
\label{addr16}
}

%
%

%
%
\thankstext[$\star$]{t1}{Corresponding authors}
\thankstext{e1}{bertoldo@mpp.mpg.de}
\thankstext{e2}{mancuso@mpp.mpg.de}



